Who are you referring to? Coreference resolution in image narrations

Coreference resolution aims to identify words and phrases which refer to same entity in a text, a core task in natural language processing. In this paper, we extend this task to resolving coreferences in long-form narrations of visual scenes. First we introduce a new dataset with annotated coreference chains and their bounding boxes, as most existing image-text datasets only contain short sentences without coreferring expressions or labeled chains. We propose a new technique that learns to identify coreference chains using weak supervision, only from image-text pairs and a regularization using prior linguistic knowledge. Our model yields large performance gains over several strong baselines in resolving coreferences. We also show that coreference resolution helps improving grounding narratives in images.

==> extra_info.tex <==
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=\linewidth]{figures/qual_results_reduced.drawio.pdf}
\vspace{-0.5cm}
\end{center}
\caption{Qualitative results of predictions on the \OurDatasetShort dataset. The colored mentions in the text indicate the ground truth coreference chains. The solid and dotted bounding boxes on the image denote the correct and incorrect localizations respectively. Below the image columns we show the predicted coreference chains. }
\label{fig:qual_results}
\end{figure}
% \vspace{-0.5em}


\noindent
\textbf{Qualitative results. }
\Cref{fig:qual_results} qualitatively analyzes CR and narrative grounding.
% trained with the combined loss function or only with contrastive loss. 
In the first two columns, we visualize the results from our proposed method. The model correctly resolves and localizes phrases such as \textit{a person, who}, \textit{the people, them} and \textit{a baby trolley, the baby trolley}. The model incorrectly grounds and chains the instance \textit{\textcolor{maroon}{a baby}}. It is interesting to note that the model pairs \textit{an object} and \textit{water sprinkler} correctly, thereby resolving ambiguity in what \textit{the object} might refer to. But it fails to add \textit{\textcolor{orange}{which}} to this coreference chain. 
It is very hard to learn coreferences for these pronouns as they come with a weak prior from language and hence are difficult for the model to disambiguate. 
Hence, we clearly show the challenging problem of coreferences we are dealing with and indicating the great potential for developing models with strong contextual reasoning. 

We also compare the performance of our method to the version trained without regularizer (Ours (w/o Reg)). 
Our final method is very effective in finding the correct coreference chains, but fails to correctly localize \textit{\textcolor{darkblue}{some of them}} and the region overlaps with \textit{\textcolor{maroon}{the people}}. 
Without regularization, it is very challenging for the model to distinguish between the instances of \textit{\textcolor{blue}{banner}} and \textit{\textcolor{magenta}{the road railing}} and hence clusters them together. Moreover, if the model has no prior imposed, it fails to correctly resolve \textit{\textcolor{blue}{behind that}}, where \textit{\textcolor{blue}{that}} refers to the \textit{\textcolor{blue}{banner in red color}}. 


\section{Detailed related work}


% \hb{don't forget Waldo, other references from the reviews, [1] Wang et.al. Improving weakly supervised visual grounding by contrastive knowledge distillation, Relation-aware Instance Refinement for Weakly Supervised Visual Grounding, CVPR 2021, Improving Weakly Supervised Visual Grounding by Contrastive Knowledge Distillation, CVPR 2021.}

% \hb{It can be good to structure here by using `paragraph'}\arushi{Done.}
% \hb{we can also refer to sup mat for some of the related work}\arushi{Good idea. I can write a more detailed related work for the supp material.}

\paragraph{Text-only CR} in NLP has a long history of rule-based and machine learning-based approaches.  
Early methods~\cite{hobbs1978resolving,raghunathan2010multi} used hand-engineered rules to parse dependency trees, which outperformed all learning-based methods at the time. 
But recently, neural network methods~\cite{wiseman2015learning, wiseman2016learning, clark2016improving, joshi2020spanbert, lee2017end} have achieved significant performance gains. 
The key idea in this work is to identify all mentions in a document using a parser and then learn a distribution over all the possible antecedents for each mention. End-to-end approaches that perform mention identification and CR together also exist. More recently, transformer models such as SpanBERT~\cite{joshi2020spanbert} incorporate a span-based masked prediction objective for pre-training and show further improvements on the downstream task of coreference resolution.
It is worth noting that all learning-based approaches require large training sets  annotated with gold standard (ground-truth) coreference chains, such as OntoNotes~\cite{pradhan2012conll} or PreCo \cite{chen2018preco}.
 

\paragraph{Visual CR} includes learning to associate people or characters mentioned in the text with images or videos \cite{ramanathan2014linking, rohrbach2017generating, cui2021s}.
Kong~\etal~\cite{kong2014you} exploit CR to relate texts to 3D scenes. 
An orthogonal direction of research is to resolve coreference in visual dialog~\cite{kottur2018visual} for developing better question-answering systems, but this is limited to specific scenarios such as linking pronouns. 
Unlike these approaches, we focus on learning coreferences from image narrations using weak supervision.

A related line of work \cite{yu2018mattnet, yu2018rethinking, li2021referring, deng2021transvg} aims to ground nouns and more complex phrases in image parts. 
In visual phrase grounding~\cite{kazemzadeh2014referitgame, yu2016modeling}, the main objective is to localize a single image region given a textual query. 
State of the art methods either use a two-stage \cite{yu2018mattnet, liu2019learning, chen2017query} method by first encoding object regions and then maximizing the similarity with the textual query or a single stage method \cite{deng2021transvg, kamath2021mdetr, li2022grounded}, where the entire image is encoded and then a localization is learned using a standard regression function to find the bounding box coordinates. 
Single stage approaches are very similar to object detection \cite{ren2015faster, he2017mask} with a conditioned text input. 
These models are trained on visual grounding datasets such as ReferItGame \cite{kazemzadeh2014referitgame}, Flickr30K Entities \cite{plummer2015flickr30k}, or RefCOCO \cite{yu2016modeling}.  
However, these methods do not ground all the words in the sentence on the images, and due to short captions
% due to the annotations' semantics 
the grounding boils down mostly to salient objects in images. Due to this limitation, grounding the words in narrations is significantly more challenging and cannot be directly be solved with off-the-shelf coreference resolution.

% Though these methods can localize a single phrase in the image (achieving up to 80\% accuracy \cite{deng2021transvg}), they fail to disambiguate coreferences (\textit{a lady} and \textit{the back side lady} that refer to different regions/entities in \Cref{fig:intro-fig}), which is the key contribution of our work.
% Few exceptions~\cite{kottur2018visual, rohrbach2017generating, huang2018finding} that can resolve coreference are limited to specific scenarios such as linking pronouns with a fixed set of characters in movies. 

% Limitations of prior image/text methods

\paragraph{Weakly supervised grounding} has recently been used in \cite{liu2019adaptive, liu2021relation, liu2019knowledge, liu2022entity, wang2021improving} for referring expression grounding with the main focus on reconstruction-based losses -- losses for language query reconstruction given the image proposal information or a consistency network where both the query and the image proposal features are reconstructed.
Other methods~\cite{wang2020maf, gupta2020contrastive, datta2019align2ground} use contrastive learning by creating many negative queries (based on word replacement) or by mining negative image regions for a given query. 
Liu \etal~\cite{liu2021relation} parses sentences to scene graph structures for capturing visual relation between entities as an auxiliary loss to improve phrase grounding. This cannot be directly integrated on our dataset, as parsing scene graphs from long narrations is typically very noisy and incomplete. 
Wang~\etal~\cite{wang2021improving} relies on regions/classes from the object detector to align phrases in the sentence but achieve this using a knowledge distillation loss. 
For fair comparison, in this paper we compare and show improvements on the MAF model \cite{wang2020maf} as it achieves comparable/better performance on Flickr30k dataset compared to \cite{liu2021relation, wang2021improving}. Furthermore, as we show in the experiments grounding is useful to anchor mentions but it is not sufficient to resolve coreferences without prior linguistic knowledge. 

% This strategy does not help in
% disambiguating multiple occurences of the same object category in the narration, a major challenge in our dataset unlike existing visual grounding datasets. 

% Our method also employs contrastive learning but for learning CR from weak supervision. 





\begin{table}[!ht]
\renewcommand*{\arraystretch}{1.13}

		\resizebox{0.9\textwidth}{!}{
			\begin{tabular}{ c c  c | c c |c }
				&  & & \multicolumn{2}{c|}{CR} & Grounding \\
				\toprule
				 Arch & Reg   & MT &  MUC-F1  & BLANC-F1 & Acc(\%)   \\ \midrule
				 \multirow{4}{*}{MLP} & \xmark   &  \xmark  &  19.9  & 66.3 & 22.74\\      
              &  \xmark  & \cmark & 18.6 & 66.0 & 24.91 \\ 
    		   & \cmark   &  \xmark  & 21.8 & 66.8 & 26.01 \\ 
		       & \cmark &  \cmark & 23.2 & 67.2 & 27.09 \\ \midrule
              \multirow{4}{*}{Tr} & \xmark   &  \xmark  & 22.2   & 66.5 & 25.97 \\
		        & \xmark   &  \cmark  & 23.3 & 67.7 & 26.75 \\ 
    		   & \cmark   &  \xmark  &  26.3 & 68.6 & 28.31 \\ 
		         & \cmark   &  \cmark  & \textbf{29.1} & \textbf{70.4} & \textbf{29.36}\\
               \bottomrule
			
\end{tabular}}
\caption{Exhaustive evaluation for our method under different settings.}
\label{table:text-trace}
\end{table}




\section{Additional Quantitative Results}

In \Cref{table:main_coref_results}, and \Cref{table:text-trace} we present an extension of results from Table 2 and Table 4 in the main paper respectively. 


More specifically, in \cref{table:main_coref_results} we add results for the MLP variant of our model architecture and the impact of regularizer on coreference resolution performance. Adding the regularization using language rules consistently improves performance in predicting correct coreference chains. 


In \cref{table:text-trace}, we evaluate the performance for both coreference resolution and grounding for different model architectures, training with/without regularization and with/without mouse traces (MT). Adding mouse traces during training improves the grounding performance significantly as it provides a very strong signal to disambiguate complex mentions better. Combination of both the mouse trace and regularizer (for both MLP and Transformer) improves on coreferencing and overall grounding accuracy.  




\begin{table*}[!ht]
\renewcommand*{\arraystretch}{1.13}

		\resizebox{0.8\textwidth}{!}{
			\begin{tabular}{c | c | c | c | c | c | c| c | c | c| c| c}

				
				
                Method & Text  & Image   & MT     & Arch & Reg & MUC-R & MUC-P & MUC-F1 & BLANC-R & BLANC-P & BLANC-F1  \\
				\toprule
			
				
			    Rule-Based \cite{lee2011stanford} & \cmark & \xmark & \xmark & - & - & 5.6 & 10.13  & 6.4 & 3.3 & 4.1  & 4.9 \\ 
			    Neural-Coref \cite{lee2017end}    & \cmark & \xmark & \xmark & - & -& 21.7 &39.4 & 24.4 & 12.0 & 58.6  & 15.5 \\  \midrule
                MAF \cite{wang2020maf}            & \cmark & \cmark & \xmark & - & -& 29.4 & 14.8 &  17.7 & 68.1 & 66.4  & 63.6 \\        \midrule
				\multirow{2}{*}{Ours}             & \cmark & \cmark & \cmark & MLP  & \xmark & 24.36 & 17.55 & 18.60 & 67.46 & 68.08 & 66.00 \\
                                                   & \cmark & \cmark & \cmark & Tr   & \xmark& 33.78  & 20.42  & 23.30 & 71.22 & 69.55 & 67.73 \\   \midrule
				     \multirow{3}{*}{Ours}   & \cmark & \cmark & \cmark & MLP  & \cmark & 35.20 &  20.08 & 23.24  & 71.72  & 69.19 & 67.25  \\
				                                      & \cmark & \cmark & \xmark & Tr   & \cmark  & 38.98 & 22.06 & 26.29 & 73.33 & 70.13 & 68.55\\ 
                                                  & \cmark & \cmark & \cmark & Tr   & \cmark & \textbf{44.11} & \textbf{24.44} & \textbf{29.13}   &  \textbf{76.34} & \textbf{71.78}  & \textbf{70.43} \\
    			  
    		\bottomrule
    			  
    			 
			
\end{tabular}}
\caption{Coreference resolution performance on the \OurDataset dataset.}
\label{table:main_coref_results}
\end{table*}

==> intro.tex <==



% Describe CR in NLP
Coreference resolution (CR) is the task of identifying all referring expressions (mentions) in a document and determining which of them refer to the same entity. 
It is a core element in many natural language processing (NLP) tasks, including question answering, document summarization, and machine translation. 
CR is a challenging problem due to the various forms that referring expressions can take in unconstrained documents.
The most common form of coreference is pronominal anaphora, where a pronoun (\eg,~\textit{she}) refers back to noun phrases earlier in the text (\eg,~\textit{the back side lady} in \Cref{fig:intro-fig}). 
Authors in~\cite{sukthanker2020anaphora} provide a recent and detailed review of CR in text data.

% Describe CR in vison+text, why can't NLP solve it, motivate its use
Despite the large body of existing work, CR research has almost exclusively focused on text data. 
However, reference to objects in a visual scene through pronouns or noun phrases commonly occurs in day-to-day speech, and often visual information is crucial for determining which pronouns, proper names, and noun phrases corefer.
In this paper, we propose a new task: multimodal coreference resolution, \ie, resolving the coreference of referring expressions in text that is paired with an image.
This form of CR is crucial for applications in multimodal reasoning, human-robot interaction, and virtual assistance. 
Aside from pronominal anaphora, phrase mentions can also corefer with other phrase mentions (\eg, \textit{a lady}, \textit{this person}, and \textit{Mary} can all refer to the same entity).
Here, we are particularly interested in identifying coreference chains with multiple mentions ($\langle$\textit{a lady, her}$\rangle$, $\langle$\textit{the back side lady, she, her}$\rangle$). 
In a visual context, we need to ground coreference chains, \ie, link them to the correct visual referent (an object bounding box), as indicated by color-coding in \cref{fig:intro-fig}. 
This even applies to singleton coreference chains (underlined in \Cref{fig:intro-fig} \eg, \textit{black hair cut sheet}).


\begin{figure}
\begin{center}
\includegraphics[width=\linewidth]{figures/fig1_reduced.drawio.pdf}
% \vspace{-0.5cm}
\end{center}
\caption{An example of coreference chain annotation from our \OurDataset dataset. Highlighted blocks of text in same color are the ground-truth coreference chains. Unlike ours, a coreference resolver from NLP \cite{lee2017end} incorrectly chains all the pronouns to \textit{the lady} (in green). For simplicity, we only show \textit{black hair cut sheet} as an example of a singleton.}
% \textit{Figure Source: Localized Narratives \cite{pont2020connecting}.}}
\label{fig:intro-fig}
\end{figure}

% why can't we use prior NLP methods
Prior CR methods~\cite{bengtson2008understanding, lee-etal-2018-higher, lee2017end, joshi2020spanbert} without image understanding are trained on annotated text and structured training data. 
For example the fact that  \textit{the first lady} can refer to \textit{Michelle Obama} can be inferred from knowledge bases \cite{vrandevcic2014wikidata, rahman2011coreference, zheng2013dynamic}. 
Also, the reference of anaphora follows clear linguistic rules \cite{lee2011stanford}, \eg, \textit{her} can refers to any female entity that appeared earlier in the text. 
However, state-of-the-art textual coreference resolvers~\cite{lee2017end, joshi2020spanbert} fail to disambiguate references correctly in our multimodal setting (as shown in \Cref{fig:intro-fig}). 
Standard image/text datasets such as COCO or Flickr30k~\cite{lin2014microsoft, krishna2017visual, changpinyo2021conceptual, plummer2015flickr30k} only contain short descriptions (typically single sentences), which include very few or no cases of coreference. 
For instance, the Flickr30k caption for the image in \Cref{fig:intro-fig} is \textit{A woman holding scissors and giving a haircut}.
These datasets therefore neither allow learning nor evaluating CR.
To address this gap, we introduce the \OurDataset, \emph{CIN} dataset, which is based on the Localized Narratives dataset~\cite{pont2020connecting}, where we augment the existing long-form descriptions with coreference chain annotation.
Furthermore, our new dataset also includes bounding box annotations, making it possible to evaluate the grounding of coreference chains. 

% In this paper, we propose to learn CR from long form narrative descriptions from paired image-text data. 
% In particular, we introduce the CRG-Flickr30k dataset which augments the existing Localized Narratives dataset \cite{pont2020connecting} with rich coreference chain annotations. Furthermore, the dataset also includes extensive bounding box annotations to evaluate grounding of coreference chains. 

Manual annotation of large datasets is expensive.
Hence we focus on learning CR from only paired image-text data under weak supervision, and use coreference chain and bounding box annotations in \OurDatasetShort only for evaluation. 
Concretely, we learn grounding mentions from paired image-text descriptions by finding the most correlated mention and image region pairs and contrasting them to the rest. 
We leverage the inferred grounding to resolve coreferring mentions by matching similar mention-region pairs.
Our method also exploits linguistic knowledge through multiple priors to favor more linguistically plausible solutions.
% Our learning objective is a combination of contrastive learning and matrix norm minimization with respect to the prior knowledge. 
We report extensive experiments on the \OurDatasetShort and demonstrate that our method not only brings significant improvements in CR but also large gains in weakly supervised visual grounding.
% \arushi{another paragraph}
% {Try to focus on high-level differences first. Aren't we using weak grounding for solving coreferencing problem rather than for sake of grounding? We use grounding to disambiguate CR? We also exploit prior knowledge from CR by encouraging recency, etc? Our method can be incorporated to visual grounding?  }


% Weak supervision


% \hb{contrast our setting to prior weakly supervised work}

% Our method
% \hb{We haven't told what our method does :)}

% Contributions
At a high-level, our work can be seen as a step towards expanding image-text understanding from single to multiple sentences. 
Our key contributions are\footnote{Our code and dataset will be made publicly available. }:
\vspace{-.2cm}
\begin{itemize}[noitemsep]
    \item a new task that aims at resolving coreferences in multimodal long form textual descriptions, 
    \item \OurDatasetShort dataset enabling the evaluation of coreference chains in text and the localization of bounding boxes in images, which is provided with multiple baselines and exhaustive analysis in multimodal CR for fostering future work,
    \item a new method that learns to resolve coreferences while jointly grounding them from weak supervision and exploiting prior linguistic knowledge,
    \item rigorous experimental evaluation showing significant improvement over the prior work not only in CR but also in weakly supervised grounding of complex phrases in long-form text, a form of disambiguation that has been underexplored in visual grounding.
\end{itemize}


% In summary, our main contributions are;

% \begin{itemize}
%     \item A novel research perspective on visual grounding by considering localization of not only noun phrases but also the pronoun phrases.  We also propose to learn to resolve the inter-linking between pronouns and nouns and other referred noun phrase expressions, popularly known as co-reference resolution in the NLP literature.
%     \item One concrete implementation of learning to localize and disambiguate phrases and resolving the co-reference links without any direct bounding box annotations or co-reference links. 
%     \item Our proposed method uniquely leverages mouse trace embeddings for the words / phrases to learn context disambiguations which is one of the unique properties of the Localized Narratives dataset. Moreover, we leverage a rule-based prior to constraint the links between co-reference during our learning process. 
%     \item We annotate bounding boxes and co-reference chains for the image-text pairs in the Flickr30k test and validation subset of the Localized Narratives dataset, which we call as the CRG-Flickr30k \footnote{CRG - Co-Reference and Grounding}. This evaluation dataset provides a benchmark for evaluating complex phrase grounding performances and a platform for research in the direction of multi-modal co-reference chain linking in free-form textual descriptions. 
%     \item (say something about analysis and experiments on dataset, problem and method.)
% \end{itemize}

==> thebigtable.tex <==
\begin{table*}[!ht]
\renewcommand*{\arraystretch}{1.13}

		\resizebox{0.8\textwidth}{!}{
			\begin{tabular}{c | c | c | c | c | c | c| c | c | c| c| c}

				
				
                Method & Text  & Image   & MT     & Arch & Reg & MUC-R & MUC-P & MUC-F1 & BLANC-R & BLANC-P & BLANC-F1  \\
				\toprule
				% VLK \cite{lu2016visual} & 8.45 & - & 3.36  & 3.75 & - & - & 3.13 & 3.52 & - & -   \\
				% VTransE \cite{zhang2017visual} & - & -  & 2.65  & 3.51 & - & - &  1.71 & 2.14 & - & -   \\
				
			    Rule-Based \cite{lee2011stanford} & \cmark & \xmark & \xmark & - & - & 5.6 & 10.13  & 6.4 & 3.3 & 4.1  & 4.9 \\ 
			    Neural-Coref \cite{lee2017end}    & \cmark & \xmark & \xmark & - & -& 21.7 &39.4 & 24.4 & 12.0 & 58.6  & 15.5 \\  \midrule
                MAF \cite{wang2020maf}            & \cmark & \cmark & \xmark & - & -& 29.4 & 14.8 &  17.7 & 68.1 & 66.4  & 63.6 \\        \midrule
				% \multirow{5}{*}{Ours}             & \cmark & \cmark & \cmark & MLP  & \xmark & 24.36 & 17.55 & 18.60 & 67.46 & 68.08 & 66.00 \\
                                                  % & \cmark & \cmark & \cmark & Tr   & \xmark& 33.78  & 20.42  & 23.30 & 71.22 & 69.55 & 67.73 \\  
				                                   % & \cmark & \cmark & \cmark & MLP  & \cmark & 35.20 &  20.08 & 23.24  & 71.72  & 69.19 & 67.25  \\
                \multirow{2}{*}{Ours}             & \cmark & \cmark & \xmark & Tr   & \cmark & &  &  &  & & \\
                                                  & \cmark & \cmark & \cmark & Tr   & \cmark & \textbf{44.11} & \textbf{24.44} & \textbf{29.13}   &  \textbf{76.34} & \textbf{71.78}  & \textbf{70.43} \\
    			  
    		\bottomrule
    			  
    			 
			
\end{tabular}}
\caption{Coreference resolution performance on the \OurDataset dataset. \textit{MT denotes mouse trace} and \textit{Tr denotes Transformer}}
\label{table:main_coref_results}
\end{table*}




\begin{table}[!ht]
\renewcommand*{\arraystretch}{1.13}

		\resizebox{0.9\textwidth}{!}{
			\begin{tabular}{ c c  c | c c |c }
				&  & & \multicolumn{2}{c|}{CR} & Grounding \\
				\toprule
				 Arch & Reg   & MT &  MUC-F1  & BLANC-F1 & Acc(\%)   \\ \midrule
				 \multirow{4}{*}{MLP} & \xmark   &  \xmark  &  19.9  & 66.3 & 22.74\\      
              &  \xmark  & \cmark & 18.6 & 66.0 & 24.91 \\ 
    		   & \cmark   &  \xmark  & 21.8 & 66.8 & 26.01 \\ 
		       & \cmark &  \cmark & 23.2 & 67.2 & 27.09 \\ \midrule
              \multirow{4}{*}{Tr} & \xmark   &  \xmark  & 22.2   & 66.5 & 25.97 \\
		        & \xmark   &  \cmark  & 23.3 & 67.7 & 26.75 \\ 
    		   & \cmark   &  \xmark  &  26.3 & 68.6 & 28.31 \\ 
		         & \cmark   &  \cmark  & \textbf{29.1} & \textbf{70.4} & \textbf{29.36}\\
               \bottomrule
			
\end{tabular}}
\caption{Coreferencing and grounding performance comparison of our method trained with and without mouse traces (MT).}
\label{table:text-trace}
\end{table}

